The Dimpled Manifold Model of Adversarial Examples in Machine Learning

The extreme fragility of deep neural networks, when presented with tiny perturbations in their inputs, was independently discovered by several research groups in 2013. However, despite enormous effort, these adversarial examples remained a counterintuitive phenomenon with no simple testable explanation. In this paper, we introduce a new conceptual framework for how the decision boundary between classes evolves during training, which we call the {\em Dimpled Manifold Model}. In particular, we demonstrate that training is divided into two distinct phases. The first phase is a (typically fast) clinging process in which the initially randomly oriented decision boundary gets very close to the low dimensional image manifold, which contains all the training examples. Next, there is a (typically slow) dimpling phase which creates shallow bulges in the decision boundary that move it to the correct side of the training examples. This framework provides a simple explanation for why adversarial examples exist, why their perturbations have such tiny norms, and why they look like random noise rather than like the target class. This explanation is also used to show that a network that was adversarially trained with incorrectly labeled images might still correctly classify most test images, and to show that the main effect of adversarial training is just to deepen the generated dimples in the decision boundary. Finally, we discuss and demonstrate the very different properties of on-manifold and off-manifold adversarial perturbations. We describe the results of numerous experiments which strongly support this new model, using both low dimensional synthetic datasets and high dimensional natural datasets.

==> 5sensitive.tex <==
\section{Why DNNs are so sensitive and humans so insensitive to adversarial perturbations}
\label{sec:philosophical}

One of the great mysteries of adversarial examples is why they are so successful even on our best trained deep neural networks, while they almost never fool the human visual system (even young babies will recognize a printed image of an adversarial cat as a cat). Our fundamental answer to this question is that through a combination of millions of years of evolution and individual experience during the first few years of life (during which the baby is only exposed to natural images), the human visual system had learned to recognize large parts of the manifold of natural images, which includes regions consisting of faces, animals, landscapes, etc. Once the visual system learns this low dimensional manifold, it can perform a projection of any given image to this manifold during its processing. For example, in all cat-like regions of the image manifold, the human visual system expects to see in a natural image certain shapes of eyes and ears, a certain form of hair texture, etc, and can correct imperfectly shaped, occluded, or cartoonishly-drawn eyes into conceptual cat-like eyes, while ignoring tiny fluctuations in individual pixel values. Similarly, when the human visual perception system encounters a handwritten $7$ digit, it does not notice the exact value of each pixel - it only records the fact that it was a $7$, and perhaps a few other distinguishing features such as whether it had a middle stroke or not, and whether the angle between the strokes was unusually sharp. It is this projection into the low dimensional image manifold during the recognition process which makes our human visual system immune to adversarial examples, since according to the new model presented here, adversarial cats differ from real cats by moving almost perpendicularly to the image manifold, and thus the projection operation eliminates any such perturbation. Notice that according to the old model of adversarial examples, an adversarial perturbation moves a cat {\it within the image manifold}, and thus the projection back to the image manifold will have no effect on the adversarial example.

This projection of a given image into the real manifold of natural images (which works so well for humans) could be our best defense against adversarial examples for future deep neural networks. However, at the moment we do not know how to define this manifold with sufficient precision. The best we can currently do is to eliminate some of the extra dimensions, which only partially removes the adversarial perturbation,  However, we believe that this promising type of defense mechanism (which had already been proposed elsewhere, e.g., in~\citet{adversarialprojdiffense} and in~\citet{meng2017magnet}) should be studied further.


==> 6experimental.tex <==
\section{Experimental results}

The main difficulty in demonstrating the correctness of the Dimpled Manifold Model is that it is not possible to directly visualize how the decision boundary looks like in a very high dimensional space. However, a simple test of this model is to measure the average distance between the training examples and the evolving decision boundary during the various training epochs. Such an experiment with the CIFAR10 dataset is described in \ref{appendix-clinging}, where the distance graph clearly shows a two phase behavior in which this distance rapidly decreases during the first few epochs as the decision boundary clings to the image manifold, and then fluctuates over many epochs without further decreases, as the dimples grow in various directions.

This characterization of the training process is further supported by an information theoretic analysis described in \citet{tishbi}. In that paper (and its accompanying video), the authors demonstrated that when they trained a DNN on a small synthetic dataset, there was a first phase in which the main effect was to increase the mutual information between the neurons in the DNN and the training inputs, and then a second phase in which the main effect was to increase the mutual information between the neurons in the DNN and the desired labels. This directly corresponds in our framework to a first phase in which the decision boundary increases its knowledge of the image manifold be clinging to it, and then a second phase in which it increases its knowledge of the labels of the training examples by creating appropriate dimples.





The dimpled manifold model is based on two testable properties. the first one (that the decision boundary passes very close to the manifold of natural images) is essentially equivalent to the statement that almost any natural image has a nearby adversarial example (which is known to be true). 
In the following sections we experimentally verify the second property (that adversarial directions are almost perpendicular to this manifold) by measuring the off-manifold and on-manifold norms of adversarial perturbations. Given a correctly classified test-set image $x$ and a local manifold $M$ around $x$, we first found an adversarial example $x+d$ (where $\norm{d}_2 \leq \epsilon$ for some small $\epsilon$, and the classifier classifies $x$ and $x+d$ differently). We then projected the adversarial perturbation $d$ onto $M$, and computed the ratio $R(d,M)$ between the norm of $d$ and the norm of its projection $d_{on}$. Note that for a random vector $r= (r_1, ... , r_{n})$ with $r_i \sim N(0,1)$ of dimension $n$, its norm is equally distributed among all the dimensions. Therefore, the expected ratio between $\norm{r}$ and $\norm{r_{on}}$ for a random vector $r$ (which we denote by $\bar{R}$) will be about $\sqrt{\frac{n}{k}}$ (see details in Appendix \ref{appendix:random-vector}). For $k<<n$ this expected ratio is large, making most vectors almost perpendicular to small manifolds by definition. 

In our experiments we measured the average of the ratio $R(d,M)$ where $d$ is an adversarial perturbation and $M$ is the natural image manifold, and compared it to $\bar{R}$ (note that values larger than $\bar{R}$ indicate actual preference of  off-manifold over on-manifold dimensions by the DNN, but any ratio larger than $\sqrt{2}$ indicates an angle larger than 45 degrees). In this paper we use the Euclidean norm in all our attacks; experiments with $L_{\infty}$-norm adversarial perturbations can be found in appendix \ref{appendix:linfinity}.


==> 7experimental_synthetic.tex <==
\section{Experiments with synthetic low-dimensional data}
In this section we demonstrate the Dimpled Manifold Model in a low-dimensional synthetic setting, in which the manifold is precisely defined, and the clinging and dimpling phases of the training can be directly visualized. We consider two illustrative settings: (1) a 1D diagonal line in a 2D input space (Figure \ref{1ddimples}) and (2) a 2D linear subspace in a 3D input space (Figure \ref{2ddimples}). In both training processes, we can see that the decision boundary is getting very close to the manifold in the first few epochs, and later a gentle dimpling process fits the given labels. In addition, it is easy to see that after the training, the adversarial directions (denoted by arrows) are roughly perpendicular to the manifold (this perpendicularity was previously observed and reported by \cite{khoury2018geometry}).\\

%These models, though quite shallow and trained over very low-dimensional data, mimic the adversarial example's behaviour of a real-life complex classifier trained over the natural image manifold. The adversarial examples are very close to any data point while doesn't resemble the adversarial class's data. \\



% \begin{figure}

% \end{figure}

% % \begin{figure}[ht!]
% %   \centering
% %  \begin{subfigure}[b]{\linewidth}
% %         \label{1ddimples}
% %   \centering
% %   \includegraphics[width=\textwidth]{images/synthetic/diagonal/cling2.PNG}
% %   %\caption{A 1D binary decision boundary evolving in a 2D input space, rapidly clinging to the 1D data manifold in the first few epochs, and slowly dimpling in the remaining epochs. The red and blue colors are the labels of the two classes. The grey lines at the specified epochs show the evolution of the decision boundary after the network is randomly initialized.}
% % \end{subfigure} \hfill

% \begin{figure}[ht!]
%         \label{1ddimples}
%   \centering
%   \includegraphics[width=\textwidth]{images/synthetic/diagonal/dimple2.png}
%   \caption{A 1D binary decision boundary evolving in a 2D input space, first clinging to the 1D data manifold then dimpling to fit the data. The red and blue colors are the labels of the two classes. The grey lines at the specified epochs show the evolution of the decision boundary after the network is randomly initialized. The last subfigure shows with arrows the adversarial directions of all the training examples after the network is fully trained, pointing roughly perpendicularly to the image manifold.}
  
%   %creates dimples. The red and blue data point belongs to different classes.  The grey lines are the levels of the model's function when random initialized and at intermediates and final epochs. In the rightmost figure we show the final decision boundary, the data points and the matching adversarial examples. The arrows represents the gradient directions from each point w.r.t to the input.}
  
%      \end{subfigure}
%      \caption{The evolution of the decision boundary over training epochs.}
% \end{figure}

% %\begin{figure}
% \label{2ddimples}
%   \centering
%   \includegraphics[width=\textwidth]{images/synthetic/diagonal/5train.PNG}
%   \caption{A 2D binary decision boundary evolving in a 3D input space, rapidly clinging to the 1D data manifold in the first few epochs, and slowly dimpling in the remaining epochs. The red and blue colors are the labels of the two classes. The grey lines at the specified epochs show the evolution of the decision boundary after the network is randomly initialized}.
  
%  % \caption{A 2D binary decision boundary clinging to the 1D data manifold and creates dimples. The red and blue data point belongs to different classes.  The grey lines are the levels of the model's function when random initialized and at intermediates and final epochs.}
% \end{figure}

% \begin{figure}
% \label{2ddimples}
%   \centering
%   \includegraphics[width=\textwidth]{images/synthetic/3D/chess/train10.PNG}
%   \caption{A 3D binary decision boundary clinging to the 2D data manifold and creates dimples. The red and blue data point belongs to different classes. Plotting the levels of the model's function when random initialized and at the end of intermediates and final epochs.}
% \end{figure}


% \begin{figure}
% \label{2ddimples}
%   \centering
%   \includegraphics[width=\textwidth]{images/synthetic/3D/diagonal/train8.PNG}
%   \caption{A 3D binary decision boundary clinging to the 1D data manifold and creates dimples. The red and blue data point belongs to different classes. Plotting the levels of the model's function when random initialized and at the end of intermediates and final epochs.}
% \end{figure}


% %\begin{figure}
% \label{2ddimples}
% \centering
% \begin{subfigure}[b]{0.3\linewidth}
% \centering
% \includegraphics[width=\textwidth]{images/synthetic/diagonal/final_adv_c.PNG}
% \caption{2D binary decision boundary, 1D data}
% \end{subfigure}
% \begin{subfigure}[b]{0.3\linewidth}
% \centering
% \includegraphics[width=\textwidth]{images/synthetic/3D/diagonal/final_adv_c.PNG}
% \caption{3D binary decision boundary, 1D data}
% \end{subfigure}
% \begin{subfigure}[b]{0.3\linewidth}
% \centering
% \includegraphics[width=\textwidth]{images/synthetic/3D/chess/final_adv_c.PNG}
% \caption{3D binary decision boundary, 2D data}
% \end{subfigure}
% \caption{A binary decision boundary of NNs, added arrows to represent gradient direction w.r.t. the input (used for adversarial attacks)}
% \end{figure}

==> 85advtrain.tex <==
\section{Adversarial training just deepen the dimples}
We look at the clinging phase as a phase induced by the data manifold, and the dimple phase as induced by the specific training data. We explain the adversarial training process using the DDM model and the aforementioned two phases. As adversarial examples are within a short distance from the data points (and therefore from the data manifold), one can assume that the clinging phase will not change due to the definition of adversarial examples as the train set. 
% In the synthetic experiments we can see this phenomena clearly \ref{cling_in_adv_train1D}, \ref{cling_in_adv_train2D}.

The major effect of the adversarial training is therefore within the dimples phase. As after the clinging phase the adversarial direction is perpendicular to the data manifold, the effect of the adversarial training on the decision boundary is a deepening of the dimples as one can see in Figure \ref{3dadvtrain}. Note, when the dimples getting deep enough, the best adversarial direction (one calculated using gradient with respect to the input) is changing. While previously the shortest way to cross the boundary was almost orthogonal to the manifold, after adversarial training the dimples is deeper, and the gradient will add a more significant on-manifold direction. However, taking a slightly larger step in the same off-manifold direction will too result an adversarial example, just a bit further. 

This conclusion help us explain why creating adversarial examples for robust networks will results a partly on-manifold examples, that does resemble the adversarial class as shown previously in \cite{ilyas2019adversarial}.

% In the synthetic setting we can see that as the dimples deepen, the gradient direction is changing. However, taking a slightly larger step in the same off-manifold direction will too result an adversarial example, just a bit further. Note, in the low dimensional setting the distance between data points from different classes is quite small in comparison to high-dimensional data. Therefore, the adversarial distance is not much smaller. However, in natural images setting adversarial step in the perpendicular direction (even through the deeper dimple) is much shorter then the distance to the natural images of the adversarial class.

% In natural images setting we train 2 classifiers - one clean and the other adversarially trained using $L_2$ one step PGD attack, and see that the adv directions are different - the second one has bigger projection over the manifold. We can also see that the adversarial direction calculated from the clean model can transfer to the robust model with slightly larger epsilon.


\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{images/synthetic/3D/chess/advtrain0-15_3.PNG}
  \caption{A 3D binary decision boundary of two NNs with the same architecture and same random initialization. The NN in the left image trained over "clean" 2D data; the right NN using adversarial training using a single-step $L_2$ PGD attack. }
  \label{3dadvtrain}

\end{figure}

% \begin{figure}
% % \label{3dadvtrain}
%   \centering
%   \includegraphics[width=\textwidth]{images/synthetic/3D/chess/advtrain0-15_3up.PNG}
%   \caption{A 3D binary decision boundary of two NNs with the same architecture and same random initialization. The NN in the left image trained over "clean" 2D data; the right NN using adversarial training using a single-step $L_2$ PGD attack. }
% \end{figure}


% \begin{figure}
% \label{2dadvtrain}
%   \centering
%   \includegraphics[width=\textwidth]{images/synthetic/3D/chess/advtrain0-15_1.PNG}
%   \caption{A 3D binary decision boundary of two NNs with the same architecture and same random initialization. The NN in the left image trained over "clean" 2D data; the right NN using adversarial training using a single-step $L_2$ PGD attack. }
% \end{figure}





==> 8experimental_natural.tex <==
\section{Experiments with natural images}
We conducted two types of experiments on each one of the MNIST, CIFAR10 and ImageNet datasets (\citet{lecun2010mnist}, \citet{CIFAR10}, \citet{IMAGENET}). For each data set, we approximated the low-dimensional natural-image manifold $M$ using an autoencoder with a high compression rate, and computed its local linearization around each test-set image $x$ (see Appendix \ref{appendix:approx-manifold} for further details and dimension specifications). This approximation may in fact overestimate $k$ (and thus underestimate the real norm ratio), yet it demonstrates well the dimpled manifold model.


\subsection{\textbf{Experiment 1: Projection of an adversarial vector}}
    For an image $x$, we started with calculating an adversarial example $x+d$ using a multi-step PGD attack (\citet{PGD}). We projected $d$ onto the locally approximated linear manifold $M$, measured the aforementioned average ratio $R(d, M) = \frac{\norm{d}}{\norm{Proj_{M}(d)}}$, and compared it to the ratio $\bar{R}$ which is expected for random vectors.
    
\paragraph{The relative effect of the projected vector on the change in classification}

To measure the effect of the on-manifold projection on the change of classification for the classifier
function $f$ (which is the neural network without the SoftMax final layer), an original class $i$, and
an adversarial class $t$, we first define the total effect of the adversarial vector $d$ as

$$
E_d = f(x'+d)_t - f(x'+d)_i - (f(x')_t - f(x')_i)
$$
    
Finally, we calculate the on-manifold relative effect out of the total adversarial effect as
    
$$
E_{Proj_M(d)} = \frac{f(x'+Proj_M(d))_t - f(x'+Proj_M(d))_i - (f(x')_t  - f(x')_i)}{E_d}
$$
    
\begin{table}[ht!]
  \caption{The norm ratio and on-manifold relative effect for natural images}
  \label{tab:natural-norm-ratio}
  \centering
  \begin{tabular}{llll}
    \toprule
    Dataset     &  $\bar{R}$     &  $R(d, M)$ & $E_{Proj_M(d)}$ \\
    \midrule
    MNIST & $\sqrt{\frac{n}{k}} = 7$  & 3.68  &  8\% \\
    CIFAR10     & $\sqrt{\frac{n}{k}} = 4.89$ & 5.59   & 4\%   \\
    ImageNet     & $\sqrt{\frac{n}{k}} = 6.48$       & 5.5 & 2\% \\
    \bottomrule
  \end{tabular}
\end{table}


In Table \ref{tab:natural-norm-ratio} one can see that for MNIST dataset the norm ratio was smaller than expected. The reason for it may be that the MNIST dataset can be successfully classified using a linear classifier, making it similar to the linear synthetic case in which the ratio was 1. Note that in all three cases, the on-manifold relative effect was tiny, demonstrating that the networks primarily used the off-manifold perturbations rather than the on-manifold perturbations in order to switch their classification.
    
In Figure \ref{fig:mnist-proj-m} and Figure \ref{fig:cifar-proj-m}, for a test-set image $x$ we show the original adversarial example $x+d$ (first row), the projected on-manifold example $x+Proj_{M}(d)$ (second row), and the projected off-manifold example $x + (d - Proj_{M}(d))$ (last row). The columns in  the figure from left to right are: the natural image $x$, the perturbed image, the perturbation itself (maximally amplifying its entries to the full range of $[0,1]$ to make it visually clearer), and the evolution of the logit's values for the various classes along the linear line $x+\alpha d$ for $\alpha \in [0, \frac{1}{100}, \frac{2}{100},...,1]$. 

\begin{figure}[ht!]
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \centering
         \includegraphics[width=\textwidth]{images/natural/mnist/mnist-proj-exmp.PNG}
       \caption{MNIST - changing 8 to 2}
    \label{fig:mnist-proj-m}

\end{figure}

In Figure \ref{fig:mnist-proj-m} we can see that the max logit is switching at $x+d$ and almost switching at the off-manifold $x + (d - Proj_{M}(d))$. However, along the linear line between $x$ and the on-manifold $x+Proj_{M}(d)$, we can see that there is almost no difference in the logits. Note that while the large off-manifold perturbation is hard to interpret, the small on-manifold perturbation is doing exactly what the human visual system would expect, trying to open the two loops in the ``8''  to get a ``2'' by blackening the relevant white segments in them.


\begin{figure}[ht!]
  \centering
         \includegraphics[width=\textwidth]{images/natural/cifar/cifar-prog-exmp.PNG}
       \caption{CIFAR10 - changing plane to ship}
    \label{fig:cifar-proj-m}

\end{figure}

In Figure \ref{fig:cifar-proj-m} we show the PGD attack and its projections on a CIFAR10 test-set image, demonstrating similar behaviour. Here, the on-manifold projection tries to change the plane visually into a ship - painting the grass in blue to resemble the sea.  Additional examples from these three datasets can be found in appendix \ref{appendix:natural-image-exam}.
    
  \subsection{\textbf{Experiment 2: Adversarial examples with on/off manifold constraints}}
    In this experiment, starting from an image $x$, we used the PGD attack with an extra constraint - before normalizing each step onto the epsilon-step sphere, we projected it on or off the approximated local linear manifold $M$ (see Appendix \ref{appendix:onoffattacks} for attack details). In this way, we generated on and off manifold adversarial examples, and compared the resultant adversarial distances between the three attacks: unconstrained PGD, on-manifold PGD and off-manifold PGD.

\begin{table}[ht!]
  \caption{The mean distance of an adversarial example}
  \label{tab:mean-distance-adv}
  \centering
  \begin{tabular}{llll}
    \toprule
    Dataset &  no-constraint PGD &  On-manifold PGD &  Off-manifold PGD \\
    \midrule
    MNIST & 1.01  & \textbf{3.68 \quad (364\%)}  &  1.05 \quad (103\%) \\
    CIFAR10     & 0.3 & \textbf{1.87 \quad (623\%)}   & 0.305 \quad (101\%)   \\
    ImageNet     & 0.149 & \textbf{0.849 \quad (570\%)} & 0.152 \quad (102\%)\\
    \bottomrule
  \end{tabular}
\end{table}

    In Table \ref{tab:mean-distance-adv} one can see a big difference in the adversarial distances. In all datasets, on-manifold adversarial examples are much further away from the original image $x$ while the off-manifold adversarial examples are much closer (up to 6 times closer). Once again, we show in Figure \ref{fig:mnist-fig} that the on-manifold adversarial perturbations are visually meaningful, while the off-manifold perturbations consist of low level noise surrounding the object's general area: At the top of Figure \ref{fig:mnist-fig} one can see that the network is creating a bird by coloring the plane and shorten its wings. Additional examples for this experiment can be found in appendix \ref{appendix:natural-image-exam}.
    
\begin{figure}[ht!]
  \centering

         \includegraphics[width=0.7\textwidth]{images/natural/onattack/cifarplanebird-n.png}

       \caption{CIFAR10 - on and off manifold attacks changing a plane into a bird}
    \label{fig:mnist-fig}

\end{figure}



==> apdix3-synthetic.tex <==
\section{Appendix - synthetic experiments}
\label{appendix:synthetic-experiments}
\subsection{Network architecture}
The experiments were conducted using the Fully-Connected network described in Figure \ref{fig:network_synth}, with the following hyperparameters:
\begin{itemize}
    \item \underline{Optimizer}: Adam
    \item \underline{Learning Rate}: 0.001
    \item \underline{Training Batch-Size}: 64
    \item \underline{Weight-Decay}: 1e-6
    \item \underline{Loss}: NLL
   
\end{itemize}

\begin{figure}[htp!]
    \centering
    \includegraphics[width=8cm]{"images/synthetic/network_structure.png"}
    \caption{Structure of the network. Input size: 3072, Number of classes: 2.}
    \label{fig:network_synth}
\end{figure}

\paragraph{CNN and FC} In this section we use Fully-Connected networks, since in our synthetic constructions nearby pixels are not correlated with each other. Convolutional networks act differently and produce different ratios since they give structures great importance: In fact, a set of input values could achieve a large norm ratio in a specific order, and a low norm ratio in a different order, whereas Fully-Connected networks typically yield the same ratio for any order of the data. With CNN and trigonometric functions in a specific order, we could easily reach norm ratios above 100, indicating an almost perfectly perpendicular direction for the perturbation.

\subsection{Technical details}
The synthetic experiments were conducted with GPU K80 using Pytorch framework (\citet{NEURIPS2019_9015}) and Numpy python-library (\citet{2020NumPy-Array}).

\subsection{The dataset generation process}
Let $n,k$ be the dimensions of the input space and the latent space respectively, and let $\mathcal{X}$ be the allowed pixels' range $[0,1]$.
\begin{enumerate}
    \item \underline{\textbf{Labels generation:}} In our experiments, we linearly partitioned the latent space into two classes, and used the nonlinearities in our trigonometric and polynomial decompression algorithms to create a complex labeling pattern on the manifold. This choice encouraged the network to learn how to map training examples back to the latent space in which determining the labels was straightforward. In all our experiments, we used the following simple partitioning of the latent space: Given $x\in\mathcal{X}^k$, we assigned it a label based on the average value of its entries:
    \[CLASS(h(x))= \begin{cases} 
          1 & Mean(x) = \frac{\sum_{j=1}^k x_j}{k}<0.5 \\
          2 & otherwise
      \end{cases}
    \]
    The label of a decompressed sample on the manifold was the same as the label given to its latent space source (note that with very high probability, no point on the manifold would be given two conflicting labels in this way).
    
    \item \underline{\textbf{First layer mapping:}}
    The first step in the sample creation process was to linearly expand the $k$ latent space coordinates into the $n$ manifold coordinates. This linear mapping $f$ had to satisfy three requirements:
    
    \begin{enumerate}
        \item To make the mapping nontrivial, each entry in the output $f(x)$ should be influenced by a large number of entries in $x$.
        \item All output entries should be within the range $[0,1]$ whenever all the input entries are within that range.
        \item The images of $f$ should be well distributed in $[0,1]^n$ rather than concentrated in a tiny subset in it (for example, a linear mapping with randomly chosen entries in $[-1,1]$ would map essentially the whole latent space cube $[0,1]^k$ into a tiny volume around the origin of the $n$-dimensional space).
    \end{enumerate}
    These considerations led us to the following choice of the linear mapping $f$. For each coordinate $1 \leq i \leq n$ in the output do the following:
    \begin{enumerate}
        \item Choose a random permutation of $k$ indices $\sigma_i$.
        \item For any input $x\in \mathcal{X}^k$ and output $y\in \mathcal{X}^n$, define $y_i$ - the output of the $i$'th coordinate for $y=f(x)$ as:
        $$y_i=\sum_{j=1}^{k'} 0.5^j\cdot (\sigma_i(x))_j$$
        where $(\sigma_i(x))_j$ is the $j$'th coordinate of $ (\sigma_i(x))$ and $k'$ is an integer between $1$ and $k$, normally $k'$ would be set to no more than $k'=10$ (since the impact of a larger number is not noticeable).
    \end{enumerate}

    \item \underline{\textbf{Second layer mapping:}}
    To create more realistic image manifolds that continuously bends within the input space, we used an additional non-linear mapping $g:\mathcal{X}^n\longrightarrow \mathcal{X}^n$ such that the full mapping from the latent space would be composed of $g\circ f$. We used two families of such second layer functions in the experiments:
    \begin{enumerate}
        \item \underline{\textbf{Trigonometric functions:}} 
        
            A vital property of $g$ is that it should be sparse in the input space. A good way of doing so is to use trigonometric functions with different numbers of cycles in each pixel, which creates a variety of high dimensional Lissajous patterns within $[0,1]^n$. Note that we should not use extremely large frequencies to prevent a random-looking mapping and numerical instability, and should not use extremely low frequencies since then the mapping will be almost linear.
            
            Define $g$ as the following function:
            \begin{enumerate}
                \item Choose randomly $n$ numbers between $BOUND_L$ to $BOUND_U$ (some reasonable numbers) to be the numbers of cycles in each coordinate in the output space, denote this vector of numbers as $frequency$.
                \item Set $phase$ to be a random vector of $n$ numbers between $0$ and $2\pi$, it would be the phase for each trigonometric function (one for each of the $n$ coordinates).
                \item For each coordinate $i$ between $1$ to $n$, define $g_i:\mathcal{X}\longrightarrow\mathcal{X}$:
                $$g_i(x) = 0.5+0.5\cdot \sin(2\pi \cdot frequency_i \cdot x+ phase_i)$$
                such that $frequency_i$ and $phase_i$ are the $i$'th elements in $frequency$ and $phase$ respectively.
                \item Finally, given $x\in\mathcal{X}^k$ from the latent space define $g:\mathcal{X}^n\longrightarrow\mathcal{X}^n$:
                $$g(x) = (g_1(f(x)_1),...,g_n(f(x)_n))$$
                where $f(x)_i$ is the $i$'th element in $f(x)$.
            \end{enumerate}
        
        \item \underline{\textbf{Polynomial functions:}}
            In this synthetic experiment, we use the same first layer mapping and the same class partitioning, but replace the trigonometric functions in the second layer mapping by a set of polynomial functions. A suitable choice of such polynomial functions is the first kind of \emph{Chebyshev polynomials} since they have the following desirable properties:
            \begin{itemize}
                \item They are polynomial mappings of arbitrarily high degrees from $[-1,1]$ to $[-1,1]$, which could be easily shifted to mappings from $[0,1]$ to $[0,1]$.
                \item Except for the first two degrees, all these polynomial functions have the same lower and upper bounds, $-1$ and $1$, respectively (unlike the second kind of \emph{Chebyshev polynomials}).
            \end{itemize}
            The \emph{Chebyshev polynomials} in this experiment had a maximum degree of \textbf{20}.

    \end{enumerate}
\end{enumerate}

\subsection{Adversarial examples as neighbors:} Since our synthetic manifold is sparse in the input space, one could claim that in these experiments, the adversarial direction is not necessarily described by the \emph{Dimpled Manifold Model}; instead, it could just point to nearby training examples from the opposite class.

A simple way to contradict this claim is to find the shortest $L_2$ distance among pairs of samples in the dataset on the one hand, and compare it to the average $L_2$ norm of  adversarial perturbations (where the adversarial perturbation is defined as the difference between a sample that classified with at least 90\% confidence level as one class, and it's adversarial example which is classified as the other class with at least  90\% confidence level.

When the average norm of adversarial perturbations is much smaller than the shortest distance among pairs of samples, it means that the adversarial example cannot be near any other sample from the dataset.

The synthetic experiment with the sparsest manifold is the one that uses trigonometric functions. We used it to test $300$ samples under two different initializations. The results of this experiment are summarized in \ref{tab:synthetic-experiments-table3}, and clearly demonstrate that adversarial examples are much closer than training examples with the opposite label.


\begin{table}[htp!]
\caption{}
  \label{tab:synthetic-experiments-table3}
  \centering
  \begin{tabular}{ c c c c}
    \toprule
 & \textbf{Network accuracy} &\textbf{Shortest distance}& \textbf{Adversarial distance} \\ 
 \midrule
 \textbf{Initialization 1} & 90\% & 25.39 & 0.55 \\  
 \textbf{Initialization 2} & 92\% & 25.48  & 0.49 \\
    \bottomrule
  \end{tabular}
\end{table}

\newpage


==> apdix7-clinging.tex <==
\section{Appendix - the clinging and dimpling phases of DNN training}
\label{appendix-clinging}
According to the Dimpled Manifold Model, during the initial phase of the training process the decision boundary should get closer to the manifold, and then it can grow shallow dimples which will have little effect on this average distance. This is clearly demonstrated in 
Figure \ref{fig:clinging}, which describes the results of training a DNN on CIFAR10 data, where the horizontal axis denotes the epoch number, and the vertical axis represents the average distance of 100 randomly chosen samples from the decision boundary at the end of each epoch (slightly overestimated by following the adversarial directions until the classification is flipped).

\begin{figure}[htp!]
    \centering
    \includegraphics[width=8cm]{"images/synthetic/clinging_phase.png"}
    \caption{During training, the decision boundary is getting closer to the manifold during the initial epochs, and then staying at roughly the same distance during later epochs}
    \label{fig:clinging}
\end{figure}

It is important to emphasize the following points:
\begin{enumerate}
\item To define a 2-class classifier, we used new labels which were the original labels modulo 2 (i.e., all the even labels were mapped to class 1, and all the odd labels were mapped to class 2). 
\item The PGD algorithm tried to flip this classification rather than to flip among the original ten classes.
\item Following that, we included all the samples regardless of whether they were misclassified after the final epoch).
\end{enumerate}


==> checklist.tex <==
%%%%% new %%%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We propose a new theoretical model which is well supported by experimental evidence but like all models it could be refined and modified in the future by new discoveries. In addition, we clearly state in the summary that we do not know how to use the new model to explain the transferability mystery of adversarial examples.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{A better theoretical understanding of the nature of adversarial examples does not seem to have any negative societal impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We enumerated all the assumptions we make and verified them experimentally.}
        \item Did you include complete proofs of all theoretical results?
\answerYes{We have only one technical lemma, for which we provide full proof in the appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We included in the appendix a full description of our experiments, which use standard software packages.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We trained synthetic classifiers and classifiers and auto-encoders on neutral image, all training details are in the appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All our experiments with natural images and synthetic data were done with standard datasets and the generation process of the adversarial examples used no randomization.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited the creators of MNIST, CIFAR10, and ImageNet datasets, and the sources of the external libraries and auto-encoders we used.}
  \item Did you mention the license of the assets?
    \answerYes{The datasets are public and so are repositories of the auto-encoders we used.}
    \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We only used standard datasets and standard computational tools in our research.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA{We did not use any data beyond the three standard datasets MNIST, CIFAR10, and ImageNet.}
\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNA{We did not use any data beyond the three standard datasets MNIST, CIFAR10, and ImageNet.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use any crowdsourcing in our research.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use any crowdsourcing in our research.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use any crowdsourcing in our research.}
\end{enumerate}


\end{enumerate}



